On Fourier analysis of polynomial multigrid for arbitrary multi-stage cycles

The Fourier analysis of the \emph{p}-multigrid acceleration technique is considered for a dual-time scheme applied to the advection-diffusion equation with various cycle configurations. It is found that improved convergence can be achieved through \emph{V}-cycle asymmetry where additional prolongation smoothing is applied. Experiments conducted on the artificial compressibility formulation of the Navier--Stokes equations found that these analytic findings could be observed numerically in the pressure residual, whereas velocity terms---which are more hyperbolic in character---benefited primarily from increased pseudo-time steps.

==> app_pmg_op.tex <==
%!TEX root = ./pmg_main.tex
\section{Additional Operator Definition for $p$-Multigrid}
\label{app:pmg}

	For the convergence of lower levels of $p$-multigrid there is a source term $\mathbf{r}_i$ that can be substituted to give the pseudo-step update equation as:
	\begin{subequations}
		\begin{align}
			\mathbf{u}_{i,n+1,m+1} =&\: \mathbf{P}_i\mathbf{u}_{i,n+1,m} - \mathbf{C}_i\sum^{s-1}_{l=0}B_{l+1}\mathbf{u}_{i,n-l} - \mathbf{K}_i\Big(\mathbf{T}_{i,0}\mathbf{u}_{i,n+1,0} + \mathbf{d}_{i} \Big) \\
			\mathbf{u}_{i,n+1,M} =&\: \mathbf{P}^M_i\mathbf{u}_{i,n+1,0} - \Bigg[\sum^{M-1}_{m=0}\mathbf{P}^m_i\Bigg]\Bigg(\mathbf{C}_i\sum^{s-1}_{l=0}B_{l+1}\mathbf{u}_{i,n-l} + \mathbf{K}_i\Big(\mathbf{T}_{i,0}\mathbf{u}_{i,n+1,0} + \mathbf{d}_{i} \Big) \Bigg)
		\end{align}
	\end{subequations}
	If we set $i=p-1$, this  leads to:
	\begin{multline}
			\mathbf{u}_{p-1,n+1,M} = \mathbf{P}^M_{p-1}\mathbf{u}_{p-1,n+1,0} - \\
			\Bigg[\sum^{M-1}_{m=0}\mathbf{P}^m_{p-1}\Bigg]\Bigg(\mathbf{C}_{p-1}\sum^{s-1}_{l=0}B_{l+1}\mathbf{u}_{p-1,n-l} + \mathbf{K}_{p-1}\Big(\mathbf{T}_{p-1,0}\mathbf{u}_{p-1,n+1,0} + \mathbf{d}_{p-1} \Big) \Bigg)
	\end{multline}
	and for compactness we will set:
	\begin{equation}
		\mathbf{S}_{p-1,M} = \sum^{M-1}_{m=0}\mathbf{P}^m_{p-1}
	\end{equation}
	Now substitutions may be made such that this update equation can be expressed in terms of the initial solution at level $p$. Hence,	
	\begin{multline}
			\mathbf{u}_{p-1,n+1,M} = \Big(\mathbf{P}^M_{p-1}\pmb{\rho}_{p-1}\mathbf{R}_{p,M} - \mathbf{S}_{p-1,M}\Big[\mathbf{K}_{p-1}\mathbf{T}_{p-1,0}\pmb{\rho}_{p-1}\mathbf{R}_{p,M} + \mathbf{K}_{p-1}\pmb{\rho}_{p-1}\mathbf{T}_{p,M}\Big]\Big)\mathbf{u}_{p,n+1,0} \\
			- \mathbf{S}_{p-1,M}\mathbf{C}_{p-1}\sum^{s-1}_{l=0}B_{l+1}\mathbf{u}_{p-1,n-l}
	\end{multline}
	This is to serve as a demonstration that the update equation at level $p-1$ can be expressed as a linear operator acting on the initial condition. However for the purposes of analytically evaluating the goings-on at each level, this nested approach will be avoided and instead values such as $\mathbf{u}_{i,p+1,0}$ and $\mathbf{d}_i$ will be made explicit.
	
	But for completeness here we will continue to finish the simple one level v-cycle. 
	\begin{multline}
		\mathbf{\Delta}_{p-1}  = - \bigg(\Big(\mathbf{P}^M_{p-1}-\mathbf{I}\Big)\pmb{\rho}_{p-1}\mathbf{R}_{p,M} - \mathbf{S}_{p-1,M}\Big[\mathbf{K}_{p-1}\mathbf{T}_{p-1,0}\pmb{\rho}_{p-1}\mathbf{R}_{p,M} + \mathbf{K}_{p-1}\pmb{\rho}_{p-1}\mathbf{T}_{p,M}\Big]\bigg)\mathbf{u}_{p,n+1,0} \\
			+ \mathbf{S}_{p-1,M}\mathbf{C}_{p-1}\sum^{s-1}_{l=0}B_{l+1}\mathbf{u}_{p-1,n-l}
	\end{multline}
